Measurement of the double beta decay half-life of Nd-150 and search for neutrinoless decay modes with the NEMO-3 detector

The half-life for two-neutrino double beta decay of Nd-150 has been measured with data taken by the NEMO 3 experiment at the Modane Underground Laboratory. The limits are also set on the half-life of different neutrinoless double beta decay of this isotope.

==> abstractschool.tex <==
\newpage
\renewcommand{\baselinestretch}{1.6}
\normalsize
\pagestyle{plain}
\begin{center}
\begin{huge}
\bf{Abstract}
\end{huge}
\end{center}
The half-life for two-neutrino double beta decay of $^{150}$Nd has been measured  with data taking by the NEMO~3 experiment at the Modane Underground Laboratory. Using $924.7$ days of data recorded with $36.55$~g of $^{150}$Nd the half-life  of this process is measured to be
\begin{equation}
T^{2\nu}_{1/2}=(9.11^{+0.25}_{-0.22}~{\rm(stat.)}\pm0.62~{\rm(syst.)})\times 10^{18}~{\rm y}.   \nonumber
\end{equation}
This result is the world's most accurate half-life measurement of this isotope. 
A search for neutrinoless double beta decay of this isotope is presented using the same data taking period. No significant excess of events above the background expectation is observed and the limit on the half-life of this process is set to be
\begin{equation}
T_{1/2}^{0\nu}>1.8\times10^{22}~{\rm y}~(90\%{\rm~CL}).      \nonumber
\end{equation}
This result has significantly improved the previous limit on neutrinoless double beta decay of this isotope. Limits are also set on several other neutrinoless double decay modes.

